Combining Automated Optimisation of Hyperparameters and Reward Shape

There has been significant progress in deep reinforcement learning (RL) in recent years. Nevertheless, finding suitable hyperparameter configurations and reward functions remains challenging even for experts, and performance heavily relies on these design choices. Also, most RL research is conducted on known benchmarks where knowledge about these choices already exists. However, novel practical applications often pose complex tasks for which no prior knowledge about good hyperparameters and reward functions is available, thus necessitating their derivation from scratch. Prior work has examined automatically tuning either hyperparameters or reward functions individually. We demonstrate empirically that an RL algorithm's hyperparameter configurations and reward function are often mutually dependent, meaning neither can be fully optimised without appropriate values for the other. We then propose a methodology for the combined optimisation of hyperparameters and the reward function. Furthermore, we include a variance penalty as an optimisation objective to improve the stability of learned policies. We conducted extensive experiments using Proximal Policy Optimisation and Soft Actor-Critic on four environments. Our results show that combined optimisation significantly improves over baseline performance in half of the environments and achieves competitive performance in the others, with only a minor increase in computational costs. This suggests that combined optimisation should be best practice.

==> tables/PPO/best_weights.tex <==
\small
\begin{tabular}{|c|c|cc|}
\hline
Reward Weight      & LunarLander & \multicolumn{1}{c|}{Ant} & Humanoid \\ \hline\hline
$w_\text{dist}$    & 3.078       & \multicolumn{1}{c|}{1.0} & 9.28     \\ \hline
$w_\text{vel}$     & 0.989       & \multicolumn{2}{c|}{-}              \\ \hline
$w_\text{tilting}$ & 0.222       & \multicolumn{2}{c|}{-}              \\ \hline
$w_\text{leg}$     & 4.53        & \multicolumn{2}{c|}{-}              \\ \hline
$w_\text{healthy}$ & -           & \multicolumn{1}{c|}{1.0} & 2.82     \\ \hline
$w_\text{force}$   & -           & \multicolumn{1}{c|}{0.5} & 0.938    \\ \hline
\end{tabular}

==> tables/SAC/best_weights.tex <==
\small
\begin{tabular}{|c|cccc|}
\hline
Reward Weight           & \multicolumn{1}{c|}{LunarLander} & \multicolumn{1}{c|}{Ant}   & \multicolumn{1}{c|}{Humanoid} & Wipe  \\ \hline\hline
$w_\text{dist}$         & \multicolumn{1}{c|}{5.901}       & \multicolumn{1}{c|}{2.253} & \multicolumn{1}{c|}{7.61}     & 7.745 \\ \hline
$w_\text{dist\_th}$     & \multicolumn{3}{c|}{-}                                                                        & 2.60  \\ \hline
$w_\text{vel}$          & \multicolumn{1}{c|}{2.691}       & \multicolumn{2}{c|}{-}                                     & 0.888 \\ \hline
$w_\text{tilting}$      & \multicolumn{1}{c|}{1.102}       & \multicolumn{3}{c|}{-}                                             \\ \hline
$w_\text{leg}$          & \multicolumn{1}{c|}{5.465}       & \multicolumn{3}{c|}{-}                                             \\ \hline
$w_\text{healthy}$      & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{0.136} & \multicolumn{1}{c|}{2.99}     & -     \\ \hline
$w_\text{force}$        & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{0.109} & \multicolumn{1}{c|}{0.916}    & 0.030 \\ \hline
$w_\text{wiped}$        & \multicolumn{3}{c|}{-}                                                                        & 82.3  \\ \hline
$w_\text{contact}$      & \multicolumn{3}{c|}{-}                                                                        & 0.594 \\ \hline
$w_\text{collision}$    & \multicolumn{3}{c|}{-}                                                                        & -83.0 \\ \hline
$\sigma$ (reward scale) & \multicolumn{1}{c|}{-}           & \multicolumn{1}{c|}{7.44}  & \multicolumn{1}{c|}{7.40}     & -     \\ \hline
\end{tabular}

==> tables/performance_external_all.tex <==
\small
\begin{tabular}{|c|cc|cccc|}
\hline
\multirow{3}{*}{Environment}                                                                  & \multicolumn{1}{c|}{\multirow{3}{*}{HPO}} & \multirow{3}{*}{RSHAPE} & \multicolumn{4}{c|}{External Objective}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \cline{4-7} 
                                                                                              & \multicolumn{1}{c|}{}                     &                         & \multicolumn{2}{c|}{PPO}                                                                                                                                                                                                                                                                & \multicolumn{2}{c|}{SAC}                                                                                                                                                                                                                                        \\ \cline{4-7} 
                                                                                              & \multicolumn{1}{c|}{}                     &                         & \multicolumn{1}{c|}{Single Obj.}                                                                                                            & \multicolumn{1}{c|}{Multi Obj.}                                                                                                           & \multicolumn{1}{c|}{Single Obj.}                                                                                                       & Multi Obj.                                                                                                             \\ \hline\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Gymnasium\\ LunarLander\\ (minimize)\end{tabular}} & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{273 $\pm$ 11\%}                                                                                                                                                                                                                                                     & \multicolumn{2}{c|}{208 $\pm$ 27\%}                                                                                                                                                                                                                             \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}424 $\pm$ 37\%\\ 287 $\pm$ 31\%\\ 242 $\pm$ 10\%\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}328 $\pm$ 30\%\\ \textbf{223 $\pm$ 10\%}\\ \textbf{207 $\pm$ 8\%}\end{tabular}}            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}188 $\pm$ 21\%\\ 175 $\pm$ 14\%\\ 174 $\pm$ 12\%\end{tabular}}                          & \begin{tabular}[c]{@{}c@{}}\textbf{179 $\pm$ 45\%}\\ \textbf{174 $\pm$ 13\%}\\ \textbf{171 $\pm$ 12\%}\end{tabular}    \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}284 $\pm$ 46\%\\ 265 $\pm$ 27\%\\ 239 $\pm$ 11\%\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}301 $\pm$ 22\%\\ 277 $\pm$ 11\%\\ 256 $\pm$ 6\%\end{tabular}}                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}202 $\pm$ 44\%\\ 194 $\pm$ 23\%\\ 191 $\pm$ 14\%\end{tabular}}                          & \begin{tabular}[c]{@{}c@{}}190 $\pm$ 36\%\\ 186 $\pm$ 15\%\\ 177 $\pm$ 11\%\end{tabular}                               \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{247 $\pm$ 30\%}\\ \textbf{234 $\pm$ 25\%}\\ \textbf{208 $\pm$ 17\%}\end{tabular}}    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}340 $\pm$ 50\%\\ 227 $\pm$ 15\%\\ 209 $\pm$ 9\%\end{tabular}}                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{185 $\pm$ 44\%}\\ 177 $\pm$ 23\%\\ \textbf{161 $\pm$ 11\%}\end{tabular}}        & \begin{tabular}[c]{@{}c@{}}191 $\pm$ 49\%\\ 182 $\pm$ 21\%\\ 170 $\pm$ 10\%\end{tabular}                               \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}360 $\pm$ 49\%\\ 262 $\pm$ 38\%\\ 211 $\pm$ 19\%\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}372 $\pm$ 62\%\\ 252 $\pm$ 24\%\\ 214 $\pm$ 8\%\end{tabular}}                              & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}194 $\pm$ 26\%\\ \textbf{171 $\pm$ 15\%}\\ 164 $\pm$ 14\%\end{tabular}}                 & \begin{tabular}[c]{@{}c@{}}196 $\pm$ 39\%\\ 193 $\pm$ 18\%\\ 174 $\pm$ 15\%\end{tabular}                               \\ \hline\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax \\ Ant\\ (maximize)\end{tabular}}      & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{6785 $\pm$ 16\%}                                                                                                                                                                                                                                                    & \multicolumn{2}{c|}{8054 $\pm$ 28\%}                                                                                                                                                                                                                            \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}6639 $\pm$ 19\%\\ 6706 $\pm$ 17\%\\ 6787 $\pm$ 13\%\end{tabular}}                            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}6307 $\pm$ 16\%\\ 6663 $\pm$ 14\%\\ 6734 $\pm$ 12\%\end{tabular}}                          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}7725 $\pm$ 33\%\\ 7927 $\pm$ 32\%\\ 7989 $\pm$ 31\%\end{tabular}}                       & \begin{tabular}[c]{@{}c@{}}7813 $\pm$ 30\%\\ 7994 $\pm$ 29\%\\ 8135 $\pm$ 23\%\end{tabular}                            \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{8011 $\pm$ 14\%}\\ \textbf{8111 $\pm$ 14\%}\\ \textbf{8214 $\pm$ 12\%}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{7728 $\pm$ 9\%}\\ 7842 $\pm$ 6\%\\ 8035 $\pm$ 4\%\end{tabular}}                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}8040 $\pm$ 23\%\\ \textbf{8264 $\pm$ 20\%}\\ 8351 $\pm$ 19\%\end{tabular}}              & \begin{tabular}[c]{@{}c@{}}\textbf{8088 $\pm$ 20\%}\\ \textbf{8216 $\pm$ 15\%}\\ \textbf{8334 $\pm$ 11\%}\end{tabular} \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}7922 $\pm$ 14\%\\ 8049 $\pm$ 12\%\\ 8172 $\pm$ 11\%\end{tabular}}                            & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}7552 $\pm$ 10\%\\ \textbf{7923 $\pm$ 6\%}\\ \textbf{8149 $\pm$ 4\%}\end{tabular}}          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{8072 $\pm$ 31\%}\\ 8199 $\pm$ 23\%\\ 8393 $\pm$ 15\%\end{tabular}}              & \begin{tabular}[c]{@{}c@{}}7582 $\pm$ 26\%\\ 8169 $\pm$ 18\%\\ 8321 $\pm$ 13\%\end{tabular}                            \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}7459 $\pm$ 22\%\\ 8013 $\pm$ 16\%\\ 8099 $\pm$ 14\%\end{tabular}}                            & \multicolumn{1}{c|}{-}                                                                                                                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}7997 $\pm$ 26\%\\ 8064 $\pm$ 21\%\\ \textbf{8470 $\pm$ 11\%}\end{tabular}}              & -                                                                                                                      \\ \hline\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax \\ Humanoid\\ (maximize)\end{tabular}} & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{4196 $\pm$ 0\%}                                                                                                                                                                                                                                                     & \multicolumn{2}{c|}{3273 $\pm$ 11\%}                                                                                                                                                                                                                            \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4287 $\pm$ 2\%\\ 4464 $\pm$ 0\%\\ 4578 $\pm$ 0\%\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4215 $\pm$ 0\%\\ 4472 $\pm$ 0\%\\ 4616 $\pm$ 0\%\end{tabular}}                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{5220 $\pm$ 17\%}\\ 5284 $\pm$ 11\%\\ 5475 $\pm$ 9\%\end{tabular}}               & \begin{tabular}[c]{@{}c@{}}4854 $\pm$ 15\%\\ 5208 $\pm$ 8\%\\ 5600 $\pm$ 1\%\end{tabular}                              \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4191 $\pm$ 6\%\\ 4826 $\pm$ 1\%\\ 5132 $\pm$ 0\%\end{tabular}}                               & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4375 $\pm$ 1\%\\ 4719 $\pm$ 0\%\\ 5038 $\pm$ 0\%\end{tabular}}                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4489 $\pm$ 20\%\\ 4881 $\pm$ 18\%\\ 5170 $\pm$ 12\%\end{tabular}}                       & \begin{tabular}[c]{@{}c@{}}4064 $\pm$ 22\%\\ 4466 $\pm$ 15\%\\ 4763 $\pm$ 4\%\end{tabular}                             \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{4844 $\pm$ 9\%}\\ \textbf{5433 $\pm$ 7\%}\\ \textbf{5661 $\pm$ 1\%}\end{tabular}}    & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{5134 $\pm$ 10\%}\\ \textbf{5485 $\pm$ 1\%}\\ \textbf{6068 $\pm$ 0\%}\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4625 $\pm$ 18\%\\ \textbf{6033 $\pm$ 12\%}\\ 6288 $\pm$ 3\%\end{tabular}}               & \begin{tabular}[c]{@{}c@{}}\textbf{5433 $\pm$ 4\%}\\ \textbf{6103 $\pm$ 1\%}\\ \textbf{6408 $\pm$ 0\%}\end{tabular}    \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4509 $\pm$ 3\%\\ 5112 $\pm$ 2\%\\ 5524 $\pm$ 0\%\end{tabular}}                               & \multicolumn{1}{c|}{}                                                                                                                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}4887 $\pm$ 20\%\\ 5913 $\pm$ 17\%\\ \textbf{6584 $\pm$ 0\%}\end{tabular}}               & -                                                                                                                      \\ \hline\hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Robosuite \\ Wipe\\ (maximize)\end{tabular}}       & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{\multirow{5}{*}{-}}                                                                                                                                                                                                                                                 & \multicolumn{1}{c|}{101 $\pm$ 24\%}                                                                                                    & \multirow{5}{*}{-}                                                                                                     \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}74 $\pm$ 34\%\\ 108 $\pm$ 24\%\\ 116 $\pm$ 20\%\end{tabular}}                           &                                                                                                                        \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}109 $\pm$ 20\%\\ 132 $\pm$ 10\%\\ 135 $\pm$ 7\%\end{tabular}}                           &                                                                                                                        \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{131 $\pm$ 11\%}\\ \textbf{136 $\pm$ 8\%}\\ \textbf{137 $\pm$ 7\%}\end{tabular}} &                                                                                                                        \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{2}{c|}{}                                                                                                                                                                                                                                                                   & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}120 $\pm$ 16\%\\ 134 $\pm$ 10\%\\ 136 $\pm$ 7\%\end{tabular}}                           &                                                                                                                        \\ \hline
\end{tabular}


==> tables/pooled_performance_external.tex <==
\small
\begin{tabular}{|c|cc|cccc|}
\hline
\multirow{3}{*}{Environment}                                                                  & \multicolumn{1}{c|}{\multirow{3}{*}{HPO}} & \multirow{3}{*}{RSHAPE} & \multicolumn{4}{c|}{External Objective}                                                                                                                                 \\ \cline{4-7} 
                                                                                              & \multicolumn{1}{c|}{}                     &                         & \multicolumn{2}{c|}{PPO}                                                                     & \multicolumn{2}{c|}{SAC}                                                 \\ \cline{4-7} 
                                                                                              & \multicolumn{1}{c|}{}                     &                         & \multicolumn{1}{c|}{Single Obj.}              & \multicolumn{1}{c|}{Multi Obj.}              & \multicolumn{1}{c|}{Single Obj.}              & Multi Obj.               \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Gymnasium\\ LunarLander\\ (minimize)\end{tabular}} & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{273 $\pm$ 11\%}                                                          & \multicolumn{2}{c|}{208 $\pm$ 27\%}                                      \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{275 $\pm$ 28\%}           & \multicolumn{1}{c|}{\textbf{228 $\pm$ 11\%}} & \multicolumn{1}{c|}{\textbf{177 $\pm$ 15\%}}  & \textbf{173 $\pm$ 22\%}  \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{261 $\pm$ 24\%}           & \multicolumn{1}{c|}{277 $\pm$ 13\%}          & \multicolumn{1}{c|}{195 $\pm$ 26\%}           & 185 $\pm$ 13\%           \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\textbf{232 $\pm$ 21\%}}  & \multicolumn{1}{c|}{\textbf{230 $\pm$ 19\%}} & \multicolumn{1}{c|}{\textbf{174 $\pm$ 25\%}}  & \textbf{179 $\pm$ 20\%}  \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{271 $\pm$ 37\%}           & \multicolumn{1}{c|}{\textbf{255 $\pm$ 27\%}} & \multicolumn{1}{c|}{\textbf{174 $\pm$ 16\%}}  & 190 $\pm$ 21\%           \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax \\ Ant\\ (maximize)\end{tabular}}      & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{6785 $\pm$ 16\%}                                                         & \multicolumn{2}{c|}{8054 $\pm$ 28\%}                                     \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{6700 $\pm$ 17\%}          & \multicolumn{1}{c|}{6614 $\pm$ 15\%}         & \multicolumn{1}{c|}{7935 $\pm$ 32\%}          & 7964 $\pm$ 28\%          \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{\textbf{8127 $\pm$ 13\%}} & \multicolumn{1}{c|}{\textbf{7852 $\pm$ 6\%}} & \multicolumn{1}{c|}{\textbf{8253 $\pm$ 21\%}} & \textbf{8176 $\pm$ 14\%} \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\textbf{8056 $\pm$ 13\%}} & \multicolumn{1}{c|}{\textbf{7916 $\pm$ 5\%}} & \multicolumn{1}{c|}{\textbf{8198 $\pm$ 23\%}} & \textbf{8128 $\pm$ 17\%} \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{7948 $\pm$ 16\%}          & \multicolumn{1}{c|}{-}                       & \multicolumn{1}{c|}{\textbf{8130 $\pm$ 21\%}} & -                        \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax \\ Humanoid\\ (maximize)\end{tabular}} & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{4196 $\pm$ 0\%}                                                          & \multicolumn{2}{c|}{3273 $\pm$ 11\%}                                     \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{4486 $\pm$ 0\%}           & \multicolumn{1}{c|}{4480 $\pm$ 0\%}          & \multicolumn{1}{c|}{5294 $\pm$ 13\%}          & 5158 $\pm$ 9\%           \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{1}{c|}{4824 $\pm$ 0\%}           & \multicolumn{1}{c|}{4709 $\pm$ 0\%}          & \multicolumn{1}{c|}{4885 $\pm$ 18\%}          & 4438 $\pm$ 16\%          \\ \cline{2-7} 
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{1}{c|}{\textbf{5312 $\pm$ 5\%}}  & \multicolumn{1}{c|}{\textbf{5419 $\pm$ 0\%}} & \multicolumn{1}{c|}{\textbf{5876 $\pm$ 12\%}} & \textbf{5759 $\pm$ 1\%}  \\ \cline{2-7} 
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{1}{c|}{5111 $\pm$ 0\%}           & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\textbf{5741 $\pm$ 12\%}} & -                        \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Robosuite \\ Wipe\\ (maximize)\end{tabular}}       & \multicolumn{2}{c|}{base}                                           & \multicolumn{2}{c|}{\multirow{5}{*}{-}}                                                      & \multicolumn{1}{c|}{101 $\pm$ 24\%}           & \multirow{5}{*}{-}       \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{2}{c|}{}                                                                        & \multicolumn{1}{c|}{103 $\pm$ 26\%}           &                          \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & base                    & \multicolumn{2}{c|}{}                                                                        & \multicolumn{1}{c|}{132 $\pm$ 10\%}           &                          \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{2}{c|}{DEHB (ours)}                                    & \multicolumn{2}{c|}{}                                                                        & \multicolumn{1}{c|}{\textbf{135 $\pm$ 9\%}}   &                          \\ \cline{2-3} \cline{6-6}
                                                                                              & \multicolumn{1}{c|}{DEHB}                 & RS                      & \multicolumn{2}{c|}{}                                                                        & \multicolumn{1}{c|}{133 $\pm$ 11\%}           &                          \\ \hline
\end{tabular}

==> tables/reward_scaling_handtuned.tex <==
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{Environment}                                                    & \multicolumn{1}{c|}{\multirow{2}{*}{HPO}} & \multirow{2}{*}{RSHAPE} & \multicolumn{2}{c|}{Handtuned Return}                    \\ \cline{4-5} 
                                                                                & \multicolumn{1}{c|}{}                     &                         & \multicolumn{1}{c|}{Implicit Scaling} & Explicit Scaling \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax\\ Ant\end{tabular}}      & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{7865 $\pm$ 2347}  & 7599 $\pm$ 2525  \\ \cline{2-5} 
                                                                                & \multicolumn{2}{c|}{DEHB}                                           & \multicolumn{1}{c|}{7956 $\pm$ 1788}  & 7714 $\pm$ 2213  \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Google Brax\\ Humanoid\end{tabular}} & \multicolumn{1}{c|}{base}                 & DEHB                    & \multicolumn{1}{c|}{11044 $\pm$ 1302} & 10508 $\pm$ 1292 \\ \cline{2-5} 
                                                                                & \multicolumn{2}{c|}{DEHB}                                           & \multicolumn{1}{c|}{11638 $\pm$ 1402} & 12141 $\pm$ 1352 \\ \hline
\end{tabular}
